Understanding In-Context Learning from Repetitions

This paper explores the elusive mechanism underpinning in-context learning in Large Language Models (LLMs). Our work provides a novel perspective by examining in-context learning via the lens of surface repetitions. We quantitatively investigate the role of surface features in text generation, and empirically establish the existence of \emph{token co-occurrence reinforcement}, a principle that strengthens the relationship between two tokens based on their contextual co-occurrences. By investigating the dual impacts of these features, our research illuminates the internal workings of in-context learning and expounds on the reasons for its failures. This paper provides an essential contribution to the understanding of in-context learning and its potential limitations, providing a fresh perspective on this exciting capability.

==> related_work.tex <==
% BACKUP !!!


\section{Related Work}
\subsection{In-Context Learning}

% Since the introduction, in-context learning has drawn extensive attention, due to its flexibility of learning any task from few demonstrations. 


% NOTE: more detailed introduction of ICL, how is that important, the key idea of analogy. 

% what previous work do, refer to the applications -> great impact !!!!!!




\paragraph{Understanding In-Context Learning.}
\cite{chan2022data} study the pretraining data and show that ICL emerges when the transformer architecture works alongside particular properties of the training data.
\cite{xie2022an} explain ICL from the perspective of Bayesian inference. They construct a synthetic dataset to prove ICL emerges when the training data follows a mixture of hidden Markov distribution. 

% \paragraph{Implicit Learning Mechanism.}
Another line of research hints that ICL performs implicit learning over demonstrations. 
\cite{garg2023transformers} propose to directly train to in-context learn the linear function and demonstrate Transformers can effectively learn unseen linear functions from in-context examples.
\cite{li2023transformers} formalize ICL as an algorithm learning problem and theoretically discuss the stability and generalization of ICL. 
\cite{hahn2023theory} derive an information-theoretic bound showing and show the compositional nature of language is the key to inducing ICL ability.

\cite{gd1,vonoswald2023transformers} demonstrate by construction and by comparison the similarity between gradient descent learner and in-context learner, and present evidence that in-context learners share algorithmic features with exact least-squares regression predictors. 
\cite{dai2023gpt} explain language models as meta-optimizers and understand in-context learning as implicit finetuning. They provide theoretical and empirical evidence to show the resemblance of the behaviors of in-context learning and explicit fine-tuning.

\elliott{update the discussion}
More related to our work, \cite{olsson2022context} introduce induction heads, that is attention heads responsible for completing sequences like [A][B] ... [A] -> [B].
They provide macro- and microscopic evidence that supports the relationship between induction head and in-context learning.  
The induction head mechanism corroborates our finding of successive reinforcement. 
Different from their work, we focus on the LLM as a whole and induction heads could potentially be a reason why token occurrence reinforcement occurs, though they have a huge gap to fill.


\paragraph{Analyzing In-Context Learning.}
Extensive work has been devoted to analyzing ICL properties. 
\cite{min2022rethinking} scrutinize four demonstrative factors that affect ICL capability: formatting tokens, label space, input distribution, and input-label mapping. Surprisingly, they find all factors except the input-label mapping matter a lot to ICL.
Contrastingly, \cite{yoo2022groundtruth} determine that the importance of input-label mapping is contingent in particular experimental settings.
Further research by \cite{wei2023larger} suggests that learning input-label mapping is an emergent ability, as revealed through their investigation of semantically unrelated ICL.
\cite{an2023incontext} emphasize that in-context demonstrations should exhibit structural similarity to the test case, diversity amongst themselves, and individual simplicity.
\cite{lu-etal-2022-fantastically} and \cite{liu-etal-2022-makes} claim the order and embedding distribution of the demonstrations crucial to the performance. 
\cite{pan2023incontext} partition the ICL ability into two subcategories, task recognition and task learning. They design controlled experiments to disentangle two subcategories and discover different phenomena when scaling model sizes. 
\cite{si2023measuring} confuse ICL ability by intentionally designing underspecified demonstrations where two possible mapping functions are available. Their findings unravel the existence of inductive biases in ICL. 

% NOTE : induction head!!!!
\elliott{We also design some settings to analyze ICL.}


\subsection{Repeating Issue and Self-Reinforcement Effect}

% Main purpose of this paragraph: First discuss why this is a notorious and severe problem in neural text generation. Then, discuss the reason of repetition. Finally, introduce self-reinforcement effect.

\paragraph{Repetition in Neural Text Generation.}

Repetition is a notorious issue in neural text generation, affecting tasks like open-ended and directed generation~\citep{holtzman2019curious,welleck2019neural,lin2021straight,see2017get,liu2019text}. Maximization-based decoding strategies lead to bland, consecutive repetitions at word, phrase, and sentence levels~\citep{holtzman2019curious,welleck2019neural,li2016simple,karpathy2015deep,guan2021long}. Despite advancements in large-scale pre-training with Transformer architecture~\citep{vaswani2017attention,radford2019language,lewis2020bart}, unexpected sentence-level repetitions persist~\citep{radford2019language, brown2020language, fu2020theoretical}. 

\paragraph{Self-Reinforcement Effect.}

The existence of the repetition issue seems weird as no such repetitive sentences in the training dataset. 
A series of research delves into the cause.
\cite{fu2020theoretical} propose a theoretical analysis, approximating language models to first-order Markov models. However, Holtzman et al.\cite{holtzman2019curious} present cases of positive feedback loops of repetitions, suggesting that repetition probability has more complicated relationships with long-range contexts, and that language models' simplification as first-order Markov models might be insufficient.
\elliott{No need to discuss so much here.}
Recently, \cite{xu2022learning} discover the \emph{self-reinforcement effect} -- a tendency for language models to assign a higher probability to the previous context sentence, and get further reinforced when the sentence occurred several times. The effect, alongside maximization decoding, gets the language model stuck into a repetitive loop. 

